MadEye: Boosting Live Video Analytics Accuracy with Adaptive Camera Configurations

Camera orientations (i.e., rotation and zoom) govern the content that a camera captures in a given scene, which in turn heavily influences the accuracy of live video analytics pipelines. However, existing analytics approaches leave this crucial adaptation knob untouched, instead opting to only alter the way that captured images from fixed orientations are encoded, streamed, and analyzed. We present MadEye, a camera-server system that automatically and continually adapts orientations to maximize accuracy for the workload and resource constraints at hand. To realize this using commodity pan-tilt-zoom (PTZ) cameras, MadEye embeds (1) a search algorithm that rapidly explores the massive space of orientations to identify a fruitful subset at each time, and (2) a novel knowledge distillation strategy to efficiently (with only camera resources) select the ones that maximize workload accuracy. Experiments on diverse workloads show that MadEye boosts accuracy by 2.9-25.7% for the same resource usage, or achieves the same accuracy with 2-3.7x lower resource costs.

==> design.tex <==
\section{Design}
\label{s:design}


- overview: Figure overviews MadEye's operation. The main insight is that PTZ cameras can rotate faster than results are needed, so we can opt for an exploration strategy that is based directly on content in different orientations, rather than purely guesses about what each orientation may have. To realize this in a way that overcomes the challenges in previous section, MadEye employs a split architecture whereby cameras employ (1) a search algorithm to determine the orientations to explore at any time (between when results are needed), and (2) a frame selection strategy to pick frames (in an informed manner) to send to the backend for full workload inference. Server inference results are continually fed back into the camera's algorithms to guide the strategies for both questions (as hints of which orientations were best and also as model updates). We describe MadEye in terms of these two components.

- Server-side
* users register queries as normal for a given scene. do they also specify an accuracy target? that seems weird since we want to boost accuracy? perhaps they just register queries
* upon registration, we train ultra-compressed, approximation model, not for the task, but just enough to determine importance of an image to that query. more specifically, how many objects of interest are there.
* describe the model architecture and training process (initialize weights using labels generated by user model on some historical dataset? this would be a blocking delay)
* then shifts to continual learning. each time server gets image and runs actual query, it will get a new, updated data point to train on. explain continual learning strategy, and when we send new model to client (just weights since arch doesn't change)
- make it clear that the models are learning to capture the per-query sensitivity in terms of model bias. client-side will deal with sensitivity in terms of query type.

- Client-side 
(1) Search module for exploring orientations
* explain the general problem framing and how it is too computationally expensive
* amorphous search (server-side does profiling of model/query sensitivity and shares that info with client; then algo is client-side and is based on local changes and gradual movement)

(2) given the images, we run the models on each considered orientation, and have workload-specific aggregation to understand the importance of orientations in terms of workload accuracy (perhaps this embeds some additional sensitivity points, e.g., via thresholds). and then we send the frames in rank order to utilize available network resources.

\subsection{Mike}
    \item Insight 1: to determine which image to send to the server, we don't actually n
\begin{itemize}

    \item We're limited on how many frames we can send for inference because of bandwidth and compute constraints
    \item To overcome this, we notice that the fast rotational speeds can enable us to explore a broad view of the region. Leverging these rotational speeds, we can take many orientations at once and only send the best one for inference.
    \item To determine this best image, we observe we can rank them based off of their relevance to the workload employ a lightweight object detection model to run on the edge to accomplish this. 
    \item Although our ranking method primarily uses count, localization is a prerequisite to getting count. While there has been prior work on ranking \cite{!!!}, not good  
    \item We use EfficientDet, a cheap object detection CNN as a lightweight proxy for each query in the workload. 
    \item EfficientDet is able to do this with a lightweight architecture because of several things: (1) we don't need the results to be perfect since they're just for ranking and (2) it is specialized for the current scene/objects; we care less about generalization

    \item We use continual learning to continuously update the model with latest data
    \item Brief overview of EfficientDet architecture and how we only train the head to improve efficiency because updating weights can take significantly longer for convergence
    \item We take weights pretrained on MS COCO and we train atop those weights using historical images from  all orientations from the current scene to fine-tune the model. We augment this training set with frames from videos that exhibit similar scenery and object compositions to help it to better generalize.
    \item These additional images help with preventing overfitting on the historical data and can lead to better generalization to scene dynamics. E.g., lighting differences in different orientations of a scene, scaling differences in objects in different parts of a scene
    \item At each epoch, we only get results back for however many images were sent to the server for inference (often times this is 1). This can result in all images coming from just several orientations, leading to catastrophic forgetting \cite{!!!}, which results in poor performance for less frequently visited orientations (which may become fruitful in the future). Since we use a compressed model, catastrophic forgetting is especially prevalent since there are fewer parameters and thus lower neural network capacity to store the requisite knowledge to perform sufficiently for a wide range of images.
    \item Tuning confidence thresholds for EfficientDet??
    \item We use each EfficientDet to estimate how each orientations fares on its corresponding query. Then we aggregate the accuracies together to get the score to rank with

Possible reasons for why generalization could help” Lighting differences in different orientations of a scene, scaling differences in objects in different parts of a scene


We have one model per query instead of per workload. One model per workload is not feasible. We’re using a cheap detection model, which coarsening space. Postprocess results to determine closeness to workload. How using coarse results and locations is sufficient. If we remove model from workload, we have to retrain workload model, but don’t have to for per-query models.

\end{itemize}


\subsection{Murali}

==> intro.tex <==
\section{Introduction}
\label{s:intro}

- Building on the steady growth in camera deployments and advances in the deep neural networks (DNNs) used to query the videos they produce (e.g., for classification or detection), live video analytics pipelines have become prevalent. These pipelines operate by continually streaming live video feeds from distributed cameras to processing servers (either edge or cloud) where DNNs are run on each frame to produce results to user-provided queries. Key use cases and applications for live video analytics include autonomous driving, footfall tracking, traffic coordination, business analytics, and surveillance.

- Given their importance, much research work has been devoted to improving live video analytics pipelines. The primary focus of recent work has been on optimizing the resource efficiency of video analytics pipelines using techniques to tune configuration knobs during inference, filter out frames, regions in frames, or entire feeds (in multi-camera settings), user cheaper model variants, and so on. But all of these works assume that the camera(s) of interest are already deployed and cannot be changed, i.e., they focus on optimizing performance for a fixed deployment.
%deployment setting is fixed, i.e., they optimize performance for an already deployed camera (or set of cameras).
%given camera deployment.
%assume that the cameras are already deployed and cannot be changed!

- Unfortunately, the deployment of video cameras for analytics is itself a daunting task for operators. Operators must pick the location of each camera, as well as its orientation (pan+tilt, i.e., rotation, and zoom) relative to the scene. Altering these decisions requires non-trivial effort, potentially involving infrastructural changes (to move cameras) or manual intervention to change orientations. Yet, prior work and our measurements suggest that query results are highly sensitive to these configuration knobs, both due to model biases regarding how objects appear in the frames, and due to scene dynamics (e.g., where objects are located). Worse, analytics pipelines typically involve diverse queries from different analysts, each of whom can focus on different objects and use different models (both in terms of architecture and weights).

%- Unfortunately, the deployment of video cameras for analytics is a daunting task for operators. Operators must pick the location of each camera, as well as its orientation (pan+tilt, i.e., rotation, and zoom) relative to the scene. Altering these decisions requires non-trivial effort, potentially involving infrastructural changes (to move cameras) or manual intervention to alter orientations. Yet, prior work and our own results show that queries/models are highly sensitive to these configuration knobs, with the best configuration varying over short time scales. Worse, the analytics performed on the generated videos (both now and in the future) can involve unforeseen queries from different analysts, highly varying models (both in terms of architectures and weights), and unpredictable changes in scene dynamics (e.g., new builds, pedestrian restrictions, traffic planning changes, etc.). \rn{something weird about timescales here: we are tuning on short time scales, but some of this sounds more like long time scales}
%Taken together, cameras represent the heart of analytics pipelines (generating the videos exposed to query platforms and analysts), but their orientations can have significant influence on analytics accuracy, with varia


- In this paper, we study whether (and how) the emerging class of PTZ (pan-tilt-zoom) cameras can be used to alleviate this burden on operators, and automatically/continually enable high-accuracy video analytics. PTZ cameras offer APIs for remote and fast tuning of orientations (e.g., rotating up to 500 degrees-per second), which in turn enable observation of any part of a 360-degree scene with different resolution and focus (based on zoom factor). Though they have been around for nearly two decades, we argue that several market trends make now the right time to explore the role they should play in video analytics: they have become very popular (global market value $>$\$3 billion in 2020), and their costs have steadily declined to being on par ($\approx$\$100) with the cheap, fixed cameras used today. Thus, they now represent a cost-effective tool that can, in the worst case, be used as fixed cameras are today. In answering the question above, we make three primary contributions. \rn{if our solution ends up being multi-pronged, we can just say that our study revealed great promise (big accuracy wins), but also key challenges: rapid tuning required, too many orientations to consider, inference/network for evaluating each. To tackle these challenges, we built MadEye. At a high level, it does online probing and it involves several key optimizations to make things practical} 

- First: dataset and analysis to understand how PTZ cameras can help. we have novel dataset that we will release, and we find that PTZ offers big opportunities. In particular, our motivational results highlight the promise of dynamically adapting those knobs to cope with dynamism in scenes and diversity in workloads: ideal tuning can result in X-Y\% accuracy improvements over \emph{the best} fixed orientation that is picked using a priori knowledge of the workload, scene, and results. \rn{something about how we study the sensitivity of different analytics queries (with diverse models, objects of interest) to these two new knobs that haven't been studied in this context: rotation and zoom}

- Second: system

- Third: evaluation 

\rn{Ravi outline ends here}

- Limitations to discuss in paper: we don't optimize for location, and instead try to do best with given location (tuning PTZ does help a bit though since we can see 360-degree scene). we also don't focus on moving cameras, and also not multi-camera
%- In this paper, we study whether (and how) the emerging class of PTZ (pan-tilt-zoom) cameras can be used to alleviate this burden on operators, and automatically enable high-accuracy, resource-aware video analytics for current and future workloads. There are a few key reasons why we want to study this: (1) PTZ cameras are rapidly growing in popularity, (2) their costs have drastically reduced, and they are now on par with the cost of cheap fixed cameras used today (e.g., \$100). Note that, in the worst case, PTZ cameras can simply be used as fixed-orientation cameras. \rn{could make this say that this paper studies the role that PTZ cameras should play to alleviate operator concerns. PTZ cameras on the surface offer the knobs and control that could tackle the static nature of the deployments today. Further, studying this now is paramount for a few reasons: PTZ cameras prevalent and cheap so no cost barrier. In studying this, we make 3-4 contributions. (1) dataset and analysis to understand how PTZ cameras can help. we have novel dataset that we will release, and we find that PTZ offers big opportunities: X-Y\% accuracy boosts. (2) system that realizes those benefits -- something about why online probing; main challenges are the massive space of orientations, network/compute delays associated with getting results during probing, and rate at which best orientation changes. solution involves lots of empirical findings. (3) eval with many queries/conditions and some realistic baselines.}

%- On the surface, PTZ cameras offer highly desirable functionality to tackle the challenges that operators currently face. In particular, they offer APIs to enable remote and fast tuning of orientations, both zoom and rotation, e.g., can rotate on the order of 200-500 degrees per second! At any point in time, they can be configured to look at any part of a 360-degree scene and with different resolution and focus (based on zoom). Further, our motivational results highlight the promise of dynamically adapting those knobs to cope with dynamism in scenes and diversity in workloads: ideal tuning can result in X-Y\% accuracy improvements over \emph{the best} fixed orientation that is picked using a priori knowledge of the workload, scene, and results.



%Camera deployments are more ubiquitous than ever in locations such as college campuses, offices, parking lots, schools, and more. Recently, we have also seen the emerging prominence of PTZ cameras which, unlike traditional static cameras, offer three additional degrees of freedom: pan, tilt, and zoom. Using these knobs, at any time instant, they can see anywhere in a 360-degree scene, and with different resolution and focus based on zoom factor. 

%The benefits of using PTZ cameras are twofold:
%\begin{enumerate}
%\item An organization can use a single PTZ camera to cover a large region, rather than needing to deploy a fleet of cameras to ensure complete coverage. This is particularly helpful as many analytics tasks don’t require continual view of the entire scene, and instead rely on coarser aggregations over longer times, or interest in certain ‘events’ that rarely happen concurrently in the entire scene.
%\item PTZ cameras obviate the need for operators to determine the ‘best’ configuration/orientation for their camera(s) a priori, and instead lets this be tuned (to a large extent) post-deployment. This is helpful because analytics tasks change over time and involve a slew of different analyst-provided models (architectures and weights) and queries, and prior work (and our own results discussed shortly) shows how orientation can affect query results.
%\end{enumerate}
To date, most prior approaches to automating PTZ camera movement has focused on tuning those knobs with the goal of tracking, i.e., following a potential object as it moves through the full scene that the PTZ camera can observe across its knob values. However, to our knowledge, the role of PTZ cameras has not been well-studied in the context of the ever-popular video analytics paradigm, whereby analytics run queries using CNNs they provide to detect/find objects of interest, their locations, classes, etc. in each frame of a live video.


% Controllable cameras includes PTZ, ePTZ, phones, drones. Two key knobs arise in all of these: rotation and zoom, both of which are not in traditional static surveillance cameras and have not been studied in the context of emerging video analytics platforms. [generally we should steer clear of discussing drones much (early at least) since that is a different animal]

% Why do people typically use controllable cameras? In the case of surveillance, I guess it's cheaper to cover a large region? The other reason is because of interest in sporadic events in different parts of a region (e.g., suspicious behavior), rather than continual coverage for, say, counting. But, we don't focus on this sporadic case in this paper.

% We focus on dynamic zoom (not optical zoom) since that is more widely deployed (e.g., cameras on phones have that) and is increasingly the common type of PTZ camera due to its lower costs. That said, our contributions generalize to other forms of zoom too.

% Perhaps the main sell should be something about cost vs. accuracy, i.e., PTZ cameras vs. fixed cameras with regards to how much monetary or resource cost there would be to achieve some analytics accuracy. Presumably, for a region, we'd need multiple fixed cameras to reach the same accuracy that we are able to get with a properly configured PTZ camera (this would be in accordance with the number of orientations we end up using). [One weird thing here is that, for a low accuracy target, only a single fixed camera may be required, and the PTZ camera may not make sense monetarily.]



% Ravi notes
- PTZ cameras have become popular: Their overall global market value has exceeded 3 billion in 2020 and is expected to steadily
grow at 2.5\% in the next years

- motivation could be based on our results. people want to run queries over regions. and today, operators deploy fixed cameras across those regions. the results thus heavily depend on where those cameras are deployed. further and unfortunately, we (and others) find that the overall results depend heavily on the orientation of cameras, the target query, objects of interest, and so on. Our goal is to enable general-purpose, high accuracy queries, so PTZ is a nice way to do that (since otherwise, it's nearly impossible to know how to configure cameras to maximize accuracy for future queries).

==> intro_var.tex <==
\section{Introduction}
\label{s:intro}

Building on the steady growth in camera deployments and advances in deep neural networks (DNNs) for vision tasks (e.g., classification or detection)~\cite{!!!}, live video analytics pipelines have become prevalent~\cite{!!!}. These pipelines operate by continually streaming live video feeds from cameras to processing servers (either edge~\cite{!!!} or cloud~\cite{!!!}), where DNNs are run on incoming frames to produce low latency and highly accurate results for different application queries, i.e., combinations of task, DNN, and object(s) of interest. Key use cases include autonomous driving, footfall tracking, traffic coordination, business analytics, among others~\cite{!!!}.

Given their practical importance, much research has been devoted to improving both the resource efficiency and accuracy of live video analytics pipelines. Existing solutions include accuracy-aware tuning of inference configuration or encoding knobs~\cite{chameleon,videostorm,accmpeg,charliepaper}, filtering out redundant content~\cite{ddns,reducto,glimpse,spatula}, employing cheaper model variants~\cite{!!!,ekya}, improving job scheduling~\cite{videstorm,nexus,gemel}, and so on. However, all of these works assume that the content captured by cameras is unchangeable, and instead can only be encoded, streamed, or analyzed differently. In essence, they focus on optimizing \emph{fixed, pre-determined} camera deployments.

Unfortunately, the deployment of cameras for analytics is itself a daunting task for operators. Subject to practical constraints (e.g., mounting poles, power sources), for a scene of interest, operators must determine the number of cameras to deploy and the orientation (i.e., a combination of rotation and zoom factor) to use for each relative to the scene. There exist many possible orientations, and altering these decisions requires manual intervention. Yet we find that doing so can be highly fruitful: across different workloads and scenes, dynamically adapting orientations over time can yield accuracy improvements of \rn{X-Y\%} (without inflating resource usage) compared to even the \emph{best} fixed-orientation scheme. Further, these wins cannot be reaped by simply deploying more fixed cameras to simultaneously cover more orientations: we find that most orientations are `best' for short periods of time (\rn{X\%} at the median), drastically hindering the efficiency of such an approach, especially in the resource-constrained settings (wireless/edge) where video analytics are run~\cite{!!!}.

An alternative strategy is to leverage PTZ (pan-tilt-zoom) cameras that offer software libraries for tuning orientations, thereby providing a logical approach to capturing the above wins. Indeed, despite existing for nearly two decades, PTZ camera popularity has surged in recent years (global market value of \$3 billion in 2020~\cite{!!!}) largely due to declining price points that now rival fixed-camera costs~\cite{!!!}. However, multiple challenges complicate their use for live analytics (\S\ref{ss:challenges}). First, queries are highly sensitive, in different ways, to orientation knobs due to their diverse goals (e.g., tasks), inherent model biases (how models perceive scenes and objects), and scene dynamism (where objects are located) -- optimizing orientation tuning for one workload can forego \rn{X-Y\%} of the potential accuracy wins for another. Second, the `grid' of orientations is large, but the selection space is sparse, with steep accuracy drops from the best orientation(s) to other at any time. Third, the best orientation changes rapidly, e.g., every \rn{X} seconds for our median workload.

%In this paper, we study whether PTZ (pan-tilt-zoom) cameras can help alleviate this burden for operators. PTZ cameras (\S\ref{ss:potential}) offer software libraries for tuning orientations and thus, on the surface, afford a logical solution for capturing the aforementioned adaptation wins. Moreover, despite existing for nearly two decades, PTZ camera popularity has surged in recent years (global market value of \$3 billion in 2020~\cite{!!!}) largely due to declining price points that now rival fixed-camera costs~\cite{!!!}. However, multiple challenges complicate their use in our setting (\S\ref{ss:challenges}). First, queries/workloads are highly sensitive, in different ways, to orientation knobs due to their diverse query goals (e.g., tasks), inherent model biases (how models perceive scenes and objects), and scene dynamism (where objects are located) -- optimizing orientation tuning for one workload can forego \rn{X-Y\%} of the potential accuracy wins for another. Second, the `grid' of orientations is large, but the selection space is sparse, with steep accuracy drops from the best orientation(s) to other at any time. Third, the best orientation changes rapidly, e.g., every \rn{X} seconds for our median workload.

To overcome these issues, we present \textbf{MadEye}, a camera-server system that automatically and continually adapts PTZ camera orientations to maximize analytics accuracy for the scene and workload at hand. The key insight behind MadEye is that the speed at which commodity PTZ cameras can change orientations (e.g., upwards of 600-degrees per second with near-instantaneous digital zoom) far outpaces the rate at which applications require analytics results (typically 1-30 frames per second (fps), i.e., every 33-1000 ms). This, in turn, allows MadEye to eschew typical non-stationary multi-armed bandit strategies~\cite{!!!} that rely purely on previous explorations to determine orientation importance, in favor of a more informed strategy based on \emph{current} scene content. Concretely, in each timestep (33 ms for 30 fps results) and subject to network/compute resource availability, MadEye cameras explore multiple orientations and quickly determine which will maximize workload accuracy and warrant transmission to the backend for full inference. However, realizing this strategy in practice involves addressing several technical challenges.

First, to enable fast camera-side evaluation of the importance of different orientations, MadEye adopts a custom transfer learning strategy with edge-grade, ultra-compressed DNN models. To cope with their potentially limited predictive power, we task them with modeling query sensitivities only to the point of accurately \emph{ranking} orientations in terms of impact on workload accuracy -- precise results are left to backend servers. Even with this relaxed framing, MadEye must employ several optimizations to achieve sufficient rank accuracy. Most notably, MadEye trains edge models using a common abstraction -- detection for objects of interest -- that reflects the minimum information needed to capture sensitivities and biases for popular tasks~\cite{!!!}. Task-specific semantics need not be baked into edge models, and instead can be incorporated by post processing the generated results.
%deferred to post processing model results.%  camera-side, and we instead defer them to the backend. %post-processing model results.

%Edge models are continually trained on MadEye's backend server using both the latest and historical workload results, with special care taken to balance data skew across recently-visited and potentially upcoming orientations.
Edge models are \emph{continually} trained on MadEye’s backend using both the latest and historical workload results, with the goal of mitigating data skew towards recently-selected orientations  (given uncertainties in what orientations will be selected next). Importantly, to balance resource costs and accuracy, each edge model covers only a single query but all orientations. The intuition is that, while model results can exhibit substantial divergence~\cite{!!!}, feature-level variance between orientations for the same scene is considerably narrower, often smaller than that in typical pre-training datasets~\cite{!!!}. Accordingly, MadEye freezes pre-trained feature extraction layers across queries, caching those weights on cameras, thereby lowering retraining and (downlink) model update overheads.

%MadEye uses a single edge model per query, but across all orientations. The intuition is that, while model results can exhibit substantial divergence~\cite{!!!}, feature-level variance between orientations for the same scene is considerably narrower, often smaller than that in typical pre-training datasets~\cite{!!!}. Accordingly, MadEye freezes pre-trained feature extraction layers across queries, caching those weights on cameras and lowering retraining and (downlink) model update overheads.

Second, we develop a novel, on-camera search strategy to explore orientations with the goal of capturing the best one (accuracy-wise) at each timestep. Three key empirical observations guide our search: (1) despite rapid temporal shifts, transitions between best orientations move slowly in the spatial dimension, (2) the best orientations are typically spatially clustered, and (3) neighboring orientations (with overlapping regions) exhibit highly correlated trends in efficacy.
% changes in best orientation often are between orientations in the same `neighborhood' (not necessarily adjacent orientations), with distant changes coming gradually.

Building on these observations, MadEye explores a flexible shape of contiguous orientations at each timestep, and considers shifting only towards neighboring orientations whose efficacy can be robustly predicted. Decisions to keep/remove orientations are governed by both response rates (and the corresponding time budgets) and \emph{relative} comparisons of recent edge model results. For the former, MadEye uses an efficient heuristic to determine path feasibility in the time budget (a variant of the NP-Hard Traveling Salesman Problem~\cite{!!!}). For the latter, MadEye gracefully trades off exploration (i.e., shape size) for network usage (i.e., sending more orientations for backend inference) to bound the effects of edge model errors and maximize accuracy for the required response rate.

%(but contiguous) shape of orientations at each timestep, expanding its shape in the next timestep only by considering neighboring orientations whose efficacy can be robustly predicted. Orientation addition/subtraction decisions are made locally, and governed by both response rates (and the corresponding time budget for exploring, transmitting, and running full workloads on orientations) and \emph{relative} comparisons from recent edge model results. For the former, MadEye employs an efficient heuristic to determine path feasibility in the time budget (a variant of the NP-Hard Traveling Salesman Problem~\cite{!!!}). For the latter, MadEye gracefully trades off exploration (i.e., shape size) for network usage (i.e., transmitting more orientations for backend inference) as edge model results grow more similar across orientations, with the goals of bounding the effects of edge model errors and maximizing accuracy for the required response rate.

Evaluating MadEye requires a dataset that supports tuning rotation and zoom at each time instant; datasets with pre-determined orientation decisions will not suffice. To our knowledge, no such dataset exists for public use, and so we developed a new corpus of PTZ-tailored videos by splicing our scenes of interest from publicly available 360-degree videos. Using this dataset, we evaluated MadEye on a variety of network conditions and workloads that incorporate multiple vision DNNs and query types: classification, counting (both per-frame and aggregate), and detection. Across these settings, MadEye  
boosts accuracy by \rn{X-Y}\% compared to an oracle fixed-orientation strategy without inflating resource usage; these wins are within \rn{X-Y}\% of the oracle dynamic strategy. Framed differently, MadEye achieves those accuracy boosts with \rn{X}$\times$ lower resource footprint compared to the best strategy of using (multiple) fixed-orientation cameras. Moreover, MadEye outperforms recent PTZ tracking algorithms~\cite{panoptes,!!!} (by \rn{X-Y}\%) and multi-armed bandit solutions~\cite{!!!} (by \rn{Y-Z}\%). We will release MadEye and our datasets post publication. \textbf{This work does not raise any ethical issues.}


%- for fixed resource usage, boosts accuracy by X-Y compared to an oracle fixed-orientation strategy, and is within X-Y of the oracle dynamic strategy.
%- framed differently, MadEye achieves those accuracy boosts with X times more efficiency compared to even the best strategy using (multiple) fixed-orientation 
%- Moreoever, MadEye outperforms recent PTZ tracking algorithms~\cite{panoptes,!!!} (by X-Y\%) and multi-armed bandit solutions~\cite{!!!} (by Y-Z\%).
%- We will release MadEye and our datasets post publication.
%- This work does not raise any ethical issues.

%- In this paper, we study if the emerging class of PTZ (pan-tilt-zoom) cameras can help alleviate this burden for operators. PTZ cameras offer APIs for remote and fast (up to 500 degrees-per-second rotation speeds) tuning of orientations. Moreover, though they have been around for nearly two decades, their popularity has surged in recent years (global market value $>$\$3 billion in 2020) largely owing to their steadily declining price points -- costs (\$100) are on par with the cheap, fixed cameras that are ubiquitous today. On the surface, PTZ cameras offer a logical solution to our problem: deploy one camera for a region and dynamically adapt its orientation based on the current workload and scene. However, the challenges above -- (1) different knob sensitivities for different queries/workloads, (2) rapidly and unpredictably changing environment, and (3) massive search space of orientations -- preclude traditional search strategies for non-stationary environments like multi-armed bandits that exhibit long convergence times, and rely purely on prior results from an orientation to determine its current importance.


%- existing solutions optimize accuracy or resource efficiency by tuning knobs, filtering frames, using cheaper models, etc. But all of these assume that the original captured content is unchangeable, and instead can only be encoded, streamed, or analyzed differently. In essence, they focus on optimizing fixed camera deployments.
%- Unfortunately, the deployment of cameras for analytics is itself a daunting task for operators. Subject to practical constraints (e.g., poles), for a scene of interest, operators must determine the number of cameras to deploy and the orientation for each (rotation and zoom relative to the scene). There exist many potential options for each knob and altering these decisions can require manual intervention. Yet we find that analytics queries are highly sensitive to both knobs due to diverse query goals (e.g., tasks), inherent model biases (how models perceive scenes and objects), and scene dynamism (where objects are located). Indeed, across many workloads and videos, we find that dynamically adapting orientations (i.e., combinations of rotations and zooms) for a scene/workload can yield accuracy improvements of X-Y\% compared to even the \emph{best} fixed-orientation scheme. [maybe mention: however, most orientations are best for short times, drastically hindering the efficiency of a deployment that simply uses many fixed cameras to cover different orientations.]
%- Unfortunately, the deployment of cameras for analytics is itself a daunting task for operators. Subject to practical constraints (e.g., poles), for a scene of interest, operators must determine the number of cameras to deploy and the orientation for each (rotation and zoom relative to the scene). There exist many potential orientations and altering these decisions can require manual intervention. Yet we find that such adaptation is fruitful: across many workloads and scenes, dynamically adapting orientations (i.e., combinations of rotations and zooms) for a scene/workload can yield accuracy improvements of X-Y\% (without inflation in resource usage) compared to even the \emph{best} fixed-orientation scheme. Further, the problem is not solved by simply deploying more cameras to simultaneously cover more orientations: we find that most orientations are `best' for short periods of time (X\% at the median), drastically hindering the efficiency of such an approach, especially in the resource-constrained settings (wireless/edge) that video analytics run~\cite{!!!}.

%- In this paper, we study if the emerging class of PTZ (pan-tilt-zoom) cameras can help alleviate this burden for operators. PTZ cameras offer APIs for rapid tuning of orientations. Moreover, though they've been around, popularity has surged largely due to declining price points (especially with ePTZ variants). On the surface, PTZ cameras offer a logical solution: deploy one camera and dynamically adapt its orientation based on the current workload and scene. However, multiple challenges complicate their use: (1) different queries/workloads are highly sensitive, in different ways, to orientation knobs due to diverse query goals (e.g., tasks), inherent model biases (how models perceive scenes and objects), and scene dynamism (where objects are located) -- optimizing for one workload can forego X-Y\% of accuracy for another; (2) the grid of orientations is large, but the selection space is sparse, with steep accuracy drops from the best orientations at a time to the others; (3) the best orientation changes rapidly (every X seconds at the median).

% challenge solution mapping
% rapid shifts: search many orientations at each timestep
% big space but sparse: empirical guidance for search algo
% sensitivity: approximation models per query


%analytics queries are highly sensitive to both knobs due to diverse query goals (e.g., tasks), inherent model biases (how models perceive scenes and objects), and scene dynamism (where objects are located). Indeed, across many workloads and videos, we find that dynamically adapting orientations (i.e., combinations of rotations and zooms) for a scene/workload can yield accuracy improvements of X-Y\% compared to even the \emph{best} fixed-orientation scheme. Moreover, the space is sparse at any time (with steep accuracy dropoffs from the best orientation) and ost orientations are best for short times, drastically hindering the efficiency of a deployment that simply uses many fixed cameras to cover different orientations.]




%Edge models are continually trained using actual workload results on shipped orientations, with special care taken to balance updating to the latest dynamics in selected orientations with preserving knowledge for other orientations that may soon be visited. Further, to keep resource costs low, each edge model is configured to operate 

%Crucially, to keep resource costs low, each edge model supports all orientations, keeping costs low. The intuition is that the variability in image features across orientations is far lower than that across images in typical pre-training detection datasets. Consequently, MadEye freezes feature extraction layers and caches the pre-trained weights on cameras. The remaining task-specific layers are used to capture per-query sensitivites, 

%* The models are continually trained and updated (only the last few layers, keeping bandwidth costs low) using only the full workload results generated by images sent to the backend while accounting for the skew in orientation data in those results (since we may visit other orientations next and want to avoid forgetting).


%* balance camera inference overheads with rank accuracy by adopting one model per query, but shared across orientations. The intuition is that pre-trained, early-stage feature extraction layers already generalize beyond the divergence in orientations for a scene; since those layers are closer to the inputs than model logic, we leave them frozen. The remaining (few) late-stage layers, on the other hand, lack the predictive power to capture the widespread biases and sensitivities of different models.


%Further, MadEye balances camera inference overheads with rank accuracy by employing an edge model per query in a workload, shared across orientations. The intuition is that pre-trained feature extraction layers generalize beyond the diversity 

%- models can't capture different algorithmic biases 



%* common abstraction of minimum info needed, i.e., detection for objects of interest --> keeps models generic (preload on camera to reduce update overhead), teases out unnecessary complexity that we can easily do with post processing (task semantics), and enables focused training whereby object-feature pairs are provided rather than simply learning these from a whole image.
%* balance camera inference overheads with rank accuracy by adopting one model per query, but shared across orientations. The intuition is that pre-trained, early-stage feature extraction layers already generalize beyond the divergence in orientations for a scene; since those layers are closer to the inputs than model logic, we leave them frozen. The remaining (few) late-stage layers, on the other hand, lack the predictive power to capture the widespread biases and sensitivities of different models.
%- Although we find limited success in matching workload results with such models, we are able to configure them to sufficiently approximate workloads by capturing their se



%To cope with the limited compute capabilities of such models, and the fact that they are tasked with capturing the sensitivities and biases of the diverse queries in a workload and for a dynamic scene, we employ several optimizations. 

%- relax to rank order problem
%- common abstraction with min sensitivity elements
%- fine-tuning with freezing
%- model per query but across orientations


%given a set of explored orientations, MadEye must determine the subset to send for remote inference, subject to both network- and compute- constraints. 

%- goal: run models on camera to determine accuracy impact of each potential orientation for current workload based on query sensitivities and scene content
%- challenge: have to use super compressed models!
%- solution: adopt a custom transfer learning strategy 

%- can't just run workload
%- adopts a transfer learning strategy whereby we use edge-grade, ultra-compressed models (called approximation models) to capture the sensitivity and biases of the current workload's queries (by training off of labeled historical data using actual model). Importantly, we relax the bar for these models by formulating the problem as a rank order one: all we need is the relative importance of each orientation for the current workload, rather than the precise results. Even then, we need several tricks to get this right:
%* common abstraction of minimum info needed, i.e., detection for objects of interest --> keeps models generic (preload on camera to reduce update overhead), teases out unnecessary complexity that we can easily do with post processing (task semantics), and enables focused training whereby object-feature pairs are provided rather than simply learning these from a whole image.
%* balance camera inference overheads with rank accuracy by adopting one model per query, but shared across orientations. The intuition is that pre-trained, early-stage feature extraction layers already generalize beyond the divergence in orientations for a scene; since those layers are closer to the inputs than model logic, we leave them frozen. The remaining (few) late-stage layers, on the other hand, lack the predictive power to capture the widespread biases and sensitivities of different models.


%orientations are largely similar in core features (same scene) --> lower discrepancies than datasets for pre-trained weights (so can just use those), and early layers are closer to image data itself (rather than model semantics), so can be shared so we freeze; then use late layers to capture model-specific semantics



%image similarity, which is less diverse than what the pre-train weights already handle
%* continually trained and updated (only the fine-tuned layer weights) using paradigm that accounts for the skew in new orientation data (since we may go to other places next, and want to avoid forgetting).

%- server: define approximation models (transfer learning to capture sensitivity and biases of each query's model but tailored -- common abstraction of objects of interest to keep models light, one model per query but shared across orientations -- insight about core feature similarity across orientations), insights in training and managing them, only need ranks (not actual query results)


%(1) Which orientations to explore?
%* note that the search is purely local, especially given rapid changes!

%(2) Which orientations to transmit?


%approx models (both design and updating)
%search (empirical observations and balancing to cope with approx errors)

%Second, we develop a novel search strategy to select orientations to explore with the goal of capturing the best one (accuracy-wise) at each timestep. Three key empirical observations guide our search: (1) despite rapid temporal shifts, transitions between best orientations move slowly in the spatial dimension, (2) the best orientations (accuracy-wise) are typically spatially clustered, and (3) neighboring orientations (with overlapping regions) exhibit highly correlated trends in efficacy.

%Building on these observations, MadEye explores an amorphous (but contiguous) shape of orientations at each timestep, expanding its shape in the next timestep only by considering neighboring orientations whose efficacy can be robustly predicted. Orientation addition/subtraction decisions are made locally, and governed by both response rates (and the corresponding time budget for exploring, transmitting, and running full workloads on orientations) and \emph{relative} comparisons from recent edge model results. For the former, MadEye employs an efficient heuristic to determine path feasibility in the time budget (a variant of the NP-Hard Traveling Salesman Problem~\cite{!!!}). For the latter, MadEye gracefully trades off exploration (i.e., shape size) for network usage (i.e., transmitting more orientations for backend inference) as edge model results grow more similar across orientations, with the goals of bounding the effects of edge model errors and maximizing accuracy for the required response rate.
%Moreoever, to rapidly compute the feasibility of each path in a given time budget (a variant of the NP-Hard Traveling Salesman Problem), MadEye employs a 





%However, to bound the effect of edge model errors and respect the required response rates (subject to network/compute resources and camera speeds), MadEye gracefully trades off exploration (i.e., shape size) with network delays (i.e., transmitting more orientations for backend inference), with the goal of maximizing accuracy per transfer.


%To respect the required response rate subject to network/compute constraints and camera properties (i.e., rotation/zoom speeds), MadEye 

%gracefully trades off exploration vs. transmissions to maximize accuracy per network transfer while respecting the required response rate.


%interesting part: use recent approximation model results, but again only relative, and use predicted error to balance exploration vs. transmissions

%- search algo: (1) temporally fast but spatially slow, (2) contiguous regions, (3) overlap --> orientations trend similarly.
%* thus, we employ a search strategy that considers an amorphous shape and only grows in a direction using neighbors where we have confidence in their utility.

%- something about efficient path selection given time budget and rotation (approximation algo with offline computations for TSM)

%- then mention balancing exploration and transmissions -- all subject to network/compute resources and camera properties -- gracefully adapts to mask approximation model errors.

%- client: search algo, rank and send, balance exploration/transmission for search with network/compute overheads and uncertainty in approximation models.

%mention that MadEye adapts its exploration vs. transmissions based on network/compute resources as well as camera properties (rotation speed). Faster networks, lower fps --> more exploration and transmission. increased sparsity in scene --> more exploration since it relies less on approximation models.

%MadEye's goal is simple: orient camera to capture orientation that will yield highest accuracy at each timestep (every 66.7 ms for 15 fps results), thereby maximizing accuracy per network usage.




%- Given their importance, much research work has been devoted to improving live video analytics pipelines. The primary focus of recent work has been on optimizing the resource efficiency of video analytics pipelines in accuracy-aware ways, using techniques to tune configuration knobs during inference, filter out frames, regions in frames, or entire feeds (in multi-camera settings), use cheaper model variants, and so on. But all of these works assume that the camera(s) of interest are already deployed and cannot be changed, i.e., they focus on optimizing performance for a fixed camera deployment, assuming that only resolution/rate of the incoming feed can be changed.

%- Unfortunately, the deployment of video cameras for analytics is itself a daunting task for operators. Subject to practical constraints (e.g., locations of mounting poles, power), operators must pick the number of cameras to deploy for a scene/region of interest, as well as the orientation for each relative to the scene, i.e., pan+tilt (rotation and zoom factor). Altering these decisions can require manual intervention, and yet we find that analytics queries are highly sensitive to both knobs due to diverse query goals, inherent model biases (how models perceive scenes and their objects), and scene dynamism (where objects are located. Worse, analytics pipelines are often run in resource-constrained wireless or edge settings with limits on power and network bandwidth (precluding the use of multiple cameras covering a region with different orientations), and are often presented with diverse queries/models that focus on different objects and use different models (architecture and weights). Some summary numbers about the problem: right orientation changes frequently for a workload (give number), varies across workloads, and not adapting foregoes X-Y\% accuracy. [You could deploy many cameras, but there are network/power constraints, and we find that this would lead to lots of wastage since orientations are often important for short periods of time.]

%- In this paper, we study if the emerging class of PTZ (pan-tilt-zoom) cameras can help alleviate this burden for operators. PTZ cameras offer APIs for remote and fast (up to 500 degrees-per-second rotation speeds) tuning of orientations. Moreover, though they have been around for nearly two decades, their popularity has surged in recent years (global market value $>$\$3 billion in 2020) largely owing to their steadily declining price points -- costs (\$100) are on par with the cheap, fixed cameras that are ubiquitous today. On the surface, PTZ cameras offer a logical solution to our problem: deploy one camera for a region and dynamically adapt its orientation based on the current workload and scene. However, the challenges above -- (1) different knob sensitivities for different queries/workloads, (2) rapidly and unpredictably changing environment, and (3) massive search space of orientations -- preclude traditional search strategies for non-stationary environments like multi-armed bandits that exhibit long convergence times, and rely purely on prior results from an orientation to determine its current importance.


%- To fill this void, we built MadEye, a system that delivers continual and resource-efficient video analytics with high accuracy. The key insight behind MadEye is that the speed at which PTZ cameras can now rotate (e.g., 400 degrees per second) far outpaces the rate at which analysts require results (often 1 FPS – see focus and other papers). This, in turn, allows MadEye to eschew the predictive approaches above and instead employ a scheme that rapidly captures a bunch of images for different orientations at a given time (i.e., between inferences), and based on their actual content, determine which are the most fruitful, i.e., which would maximize accuracy for a given workload and bandwidth availability. Concretely, MadEye consists of two key components that embed several new strategies to realize this strategy in practice. 

%- We develop new strategies to determine what orientations to consider at any time given the fast, but restricted, rotation speed of PTZ cameras. Two key principles guide our search. First, we observe that, although the best orientation can change rapidly over time, those transitions are often slow-moving spatially. In other words, changes in best orientation often are between orientations in the same `neighborhood' (not necessarily adjacent orientations), with distant changes coming gradually. MadEye thus employs an amorphous region for its search area at any time: keeps the set of orientations relatively stable across seconds, but willing to move *gradually* in different directions.

%- Second, we conduct a study to unearth the model-, query-, and object-type sensitivities to rotation/zoom knobs. We find several interesting things, e.g., compressed models require more zoom, coarser queries are less sensitive, etc. However, more importantly, we find that these characteristics can be gleaned from quick, one-time profiling of a model/query. MadEye thus infers this information once, as queries are registered, and balances these per-query insights to guide its search in favor of maximizing overall (i.e., across the workload) accuracy. [easy way to say this: the sensitivity results tell us how to shape the amorphous region at any time, i.e., how much to explore in any one direction. And the search is slow in that direction since we find that changes are generally nearby.]

%- Given a set of images from different orientations at any time, MadEye must then select the subset to send to the remote (edge or cloud) server for workload inference, subject to both network and on-camera processing constraints. The goal is to maximize accuracy per byte, i.e., send the most fruitful images. Moreover, we cannot simply run the whole workload on the camera, and instead are restricted to small/compressed models. To make the most out of these limited models, we turn to continual learning to limit how much generality we ask of the model. However, even that is not enough: compared to prior continual learning strategies, our problem is harder (ranking the importance of images for a workload, rather than simply classifying pre-determined bounding boxes).

%- Our key insight is to structure this task as a simpler problem for the model: don't use a ranker that takes in a bunch of images, and instead use the model to predict counts (since queries are object centric, we find that count is a good proxy for diverse queries) for each image alone, and then rank based on those counts. note that we don't need perfect counts; just enough to get the right rankings. We choose this because loss functions for tasks like counting are much easier to use than those for ranking (why??). Moreover, we opt to use an ultra-compressed model to represent each query (since models can perceive the same object type differently), i.e., one tiny model aims to predict the count of objects relevant to a given query/model -- cameras today can run many of these in parallel. These models are trained periodically using the real workload results only for images that are actually sent to the backend (so there is no additional full-workload inference that we are introducing)

%- Evaluating PTZ cameras requires a dataset that allows the tuning of rotation and zoom at every time instant, i.e., we cannot use a dataset that is based on specific rotation/zoom decisions, and instead need the ability to tune those knobs ourselves. To our knowledge, such a dataset does not exist. So, we created one using publicly available 360-degree videos. We divided them into an overlapping grid (to mimic a continual rotation space), and enable zoom using ??? 

%- Using this dataset, we evaluated MadEye on a variety of deep learning models and query types: classification, counting (both per frame and aggregate), and detections, as well as different network conditions. Across these scenarios, MadEye is consistently and continually able to meet accuracy targets. Specifically, MadEye achieves X-Y\% accuracy boosts compared to the (impractical) best fixed camera approach; results are Y-Z\% relative to the unachievable best PTZ approach. More practically, accuracy boosts are Y-Z\% and Z-Y\% relative to existing PTZ tracking algorithms, and Z\% over generic multi-armed bandwidth searches. Framed differently, to achieve the same accuracy, MadEye requires Y-Z\% fewer cameras and bandwidth relative to the best possible approach of deploying fixed cameras. We will open source. [could also tease out whole scene and aggregate stuff as things that become more reaslistic with PTZ] \rn{perhaps another win is reducing the amount of content that is sent without being best? something about resource usage is good, e.g., X times lower resource overhead for same accuracy} \rn{This work does not raise any ethical issues.}

%In summary, our contributions are:
%- sensitivity study to this emerging class of knobs
%- Madeye, system that efficiently and automatically explores regions using PTZ cameras to enable high-accuracy analytics under bandwidth constraints, thereby simplifying the camera deployment challenge for operators. MadEye uses a novel continual learning strategy to guide its search.
%- A thorough evaluation of MadEye with different models/queries, and a new dataset (which is required when considering rotation/zoom) that we will release.


\begin{comment}
_______intro notes______

maybe this should really just focus almost entirely on small regions (wanting to do analytics on an intersection or a part of a street): even in that small area, there are tons of orientations. objects move and models are sensitive, and so a fixed camera will surely miss many things (since the right orientation will vary over time). PTZ lets you cover that area with just one camera.
* and then we can say, this naturally extends to broader scenes (the results scale as expected), and also the wins grow for other types of queries like aggregate counting
* for a small region, how many orientations are there? 


we are improving accuracy per bandwidth: you would have to deploy many fixed cameras to cover important regions and orientations, but 

you could deploy tons of fixed cameras, but then you'd still have the challenge of figuring out which set of frames to send to best use available bandwidth! Each can do local computations, but that is not enough.
\end{comment}

==> methodology.tex <==
\section{Background and Methodology}
\label{s:methodology}

In this section, we provide a background of video analytics pipelines and controllable cameras. We also discuss the curation of our video dataset.

\subsection{Video Analytics and Controllable Cameras}
Cities and large organizations are becoming increasingly dependent on camera deployments to continuously monitor locations such as college campuses, homes, factories, and more. Along with the surge in camera usage, video analytics have risen in popularity to automatically analyze video frames for a plethora of different important functions such as security surveillance and traffic monitoring. In these live video analytics pipelines, cameras stream video frames to servers that execute computer vision models on them, which are typically placed on cloud servers, edge servers, or even directly on the cameras themselves. Privacy is also a concern and can push processing to the edge. The goals of these systems platforms running video analytics are to take in models and queries from users, and generate high accuracy and low latency results. Users may specify an accuracy target for the query and can restrict processing to be done on only a subset of frames to focus on a specific time range. For instance, an operator can issue a query to get the number of cars on the road to gauge traffic congestion at specific times of the day. 

Traditionally, video analytics pipelines have focused on static cameras (e.g., \cite{!!!}) and prior work on studying video analytics in the context of \textit{controllable cameras} has been comparatively sparse. Controllable cameras provide operators with the freedom to control a set of \textit{knobs} that modify the camera's field-of-view. For instance, PTZ cameras \cite{ptzoptics-cameras,sony-srg-300h}, which have been skyrocketing in popularity \cite{ptz-camera-market}, are motorized cameras that enable operators to pan (i.e., horizontal rotation), tilt (i.e., vertical rotation), and zoom. ePTZ cameras \cite{!!!} are also becoming increasingly prominent and provide a cheaper alternative to traditional PTZ cameras by capturing large 4k videos and allowing the operator to electronically pan, tilt, and zoom into those 4k feeds. Further examples include drones and phones which, unlike stationary PTZ and ePTZ cameras, introduce movement that dynamically changes the scene. To better discuss and compare the effects of the knobs, we define the \textit{orientation} of a camera as a specific configuration of the camera knobs that yields a unique view of the scene. In this paper, we focus on pan, tilt, and zoom knobs. For simplicity, we use \textit{rotation} to refer to both pan and tilt.

\subsection{Dataset Creation}

\Para{Dataset collection methodology.} To study the integration of controllable cameras in video analytics pipelines, we require a video dataset that mimics the effects of tuning controllable camera knobs. To the best of our knowledge, there are no controllable camera datasets that are of public settings (e.g., college campuses and traffic intersections) that offer the flexibility to remotely control those knobs. While there are exist several PTZ video datasets available (e.g., \cite{ski-ptz-dataset}), they are short (several minutes of video feed), scarce, and only consist of PTZ video feeds already in a previously-selected orientation so other orientations cannot be explored. 


Thus, we instead build a dataset that consists of camera feeds from many different orientations to faithfully mimic the effects of the PTZ camera knobs. We do this by downloading existing 360-degree videos from Youtube and extracting a video feed for each possible orientation. For a given video, we use 216 different orientations at different pan, tilt, and zoom levels. The pan orientations comprehensively cover the entire 360-degree space which is akin to PTZ cameras that can pan up to 340 degrees \cite{understainding-eptz-ptz}. While PTZ cameras can tilt to a maximum of 120 degrees, we find that the vast majority of objects in our videos cannot be detected at tilt orientations past 30-degrees downwards or upwards since those frames capture the ground and sky respectively, so we offer a maximum tilt of 60 degrees which is also representative of ePTZ camera tilt limits \cite{ptz-eptz-difference}. In simulating zoom, we first note that many existing PTZ cameras use optical zoom \cite{optical-zoom} which leverages the physical change in the camera lens to adjust the distance between the sensor and object thus maintaining image quality. Since we use existing 360-degree video, we do not have the option of using optical zoom and hence use digital zoom \cite{digital-zoom}, which involves cropping the image and scaling the dimensions back to its original size. Because we are using existing videos, we cannot use optical zoom and we instead use digital zoom. Although digital zoom does degrade the resolution of the image, our approach still reflects the zoom capabilities of many cameras (e.g., ePTZ cameras \cite{!!!}). We currently use zoom factors of 1x, 2x, and 3x which are the zoom settings that many ePTZ users opt for due to the resolution degradation for higher factors -- a 4K frame that is magnified by 3x results in a degradation to 720p \cite{understainding-eptz-ptz}. Note that our dataset creation platform offers users the flexibility to generate further orientations (e.g., beyond 3x zoom or increasing the maximum tilt) than the ones we use if needed.

\Para{Videos.} Our dataset consists of over 10 total hours of video feed taken from 10+ 360-degree videos scraped from Youtube. Because of our requirement that the video feeds not only contain target objects of interest (i.e., either people or cars), but also be stationary to mimic the deployment settings of PTZ cameras, our video selection is constrained. Further, there's a computational constraint for our analysis since we have to run coordinate conversion, model inference, and query execution for all orientations on each frame.  Because each one of our videos features a different setting, our dataset exhibits a variety of different object densities, object sizes, and lighting. These videos include crowded streets, traffic intersections, highways, marketplaces, indoor shopping centers, and more.


\subsection{Models and Tasks}  We consider 4 popular computer vision models frequently used in recent literature: (1) SSD \cite{ssd} with ??? backbone trained on Pascal VOC \cite{Everingham:2010:PVO:1747084.1747104}, YOLOv4 \cite{yolov4} with CSPDarknet53 backbone trained on MS-COCO\cite{lin2015microsoft} \cite{yolov4}, Tiny YOLOv4 \cite{yolov4} with CSPDarkNet53 backbone trained on MS-COCO, and Faster RCNN \cite{faster-rcnn} with ResNet-50 backbone trained on MS-COCO. SSD was trained on Pascal VOC \cite{Everingham:2010:PVO:1747084.1747104} and the rest were trained on MS-COCO \cite{lin2015microsoft}. 
 The tasks/queries our selected models consist of (in decreasing order of coarseness) (1) binary classification for determining whether an object is in the scene, (2) counting to get the number of objects in a scene, (3) object detection which detects all instances of an object and draws bounding boxes around them, and (4) aggregate counting of unique objects over a temporal window. In this paper, we focus on cars and people as the objects of interest for our binary classification, counting, and mAP tasks because of their use in recent literature and importance in many existing video analytics queries.  \cite{!!!}. Because many of the car videos in our dataset contain a choke point that all cars pass through (and can be captured in a single orientation), we only focus on people for aggregate counting. To prevent overcounting for our aggregate counting, we use ByteTrack \cite{bytetrack}, an existing multi-object tracker.




%ravi note: PARSEC paper has nice short description of 360-degree videos and equirectangular projection

==> motivation.tex <==
\section{Motivation}
\label{s:motivation}



% Results across a bunch of videos, models, and queries highlighting the following for zoom and rotation knobs:
% - models are sensitive to the knobs
% - sensitivity varies across models (and scenes/query types)
% - sensitivity varies across query types
% - sensitivity varies across objects of interest
% - zoom and rotate help beyond just bringing new objects into the scene (particularly with rotations). one key aspect is the orientation and size of the object in the scene -- prior work has shown these aspects to dramatically affect model accuracy, e.g., small objects are often missed!

\begin{figure}[!t]
  \includegraphics[width=\columnwidth]{figures/binary.pdf}
 \caption{Binary classification accuracy comparisons between the best fixed and dynamic orientation.}
 \label{fig:binary-classification}
 \end{figure}
 
 \begin{figure}[!t]
  \includegraphics[width=\columnwidth]{figures/count.pdf}
 \caption{Counting accuracy comparisons between the best fixed and dynamic orientation.}
 \label{fig:count}
 \end{figure}
 
  \begin{figure}[!t]
  \includegraphics[width=\columnwidth]{figures/detection.pdf}
 \caption{Detection accuracy score comparisons between the best fixed and dynamic orientation.}
 \label{fig:detection}
 \end{figure}
 
  \begin{figure}[!t]
  \includegraphics[width=\columnwidth]{figures/aggregate.pdf}
 \caption{Aggregate counting accuracy comparisons between the best fixed and dynamic orientation.}
 \label{fig:aggregate-count}
 \end{figure}
 
  \begin{figure}[!t]
  \includegraphics[width=\columnwidth]{figures/cdf.pdf}
 \caption{CDF showing the distribution of durations in seconds that an orientation remains optimal for 4 different videos.}
 \label{fig:duration-cdf}
 \end{figure}
 
 
 
\begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/rotation-unseen1.jpg}
 \label{fig:rotation1a}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/rotation-seen1.jpg}
  \label{fig:rotation1b}
\end{subfigure}
\caption{Two images showing how more objects are found when the camera is rotated to the left.}
\label{fig:rotation1}
\end{figure}



\begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/rotation-unseen2.jpg}
 \label{fig:rotation2a}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/rotation-seen2.jpg}
\label{fig:rotation2b}
\end{subfigure}
\caption{Images showing that rotation can affect whether an object can be detected or not despite it being visible in both frames. In this example, the van cannot be identified in the first frame but can be detected in the second.}
\label{fig:rotation2}
\end{figure}


\begin{figure}
\centering
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/rotation-unseen3.jpg}
 \label{fig:rotation3a}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/rotation-seen3.jpg}
    \label{fig:rotation3b}
\end{subfigure}
\caption{Two images showing the same orientation a minute apart, showing how how object densities change over time.}
\label{fig:rotation3}
\end{figure}



 \begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/zoom-unseen1.jpg}
    \label{fig:zoom1a}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.98\textwidth]{figures/zoom-seen1.jpg}
  \label{fig:zoom1b}
\end{subfigure}
\caption{Two images showing how zoom can be activated to detect faraway cars.}
\label{fig:zoom1}
\end{figure}
 
 
\begin{figure}[!t]
  \includegraphics[width=\columnwidth]{example-image-a}
 \caption{Differences in accuracy when considering 4 different workloads.}
 \label{fig:workload}
 \end{figure}
 
\begin{figure}[!t]
  \includegraphics[width=\columnwidth]{example-image-a}
 \caption{Degradation in accuracy per workload when using fixed versus dynamic orientations. We plot a bar chart showing the accuracy of a workload. The height of the bar represents the median across different videos.}
 \label{fig:workload}
\end{figure} 
 
\subsection{Importance of camera knobs.}
The performance of computer vision models running in video analytics pipelines is highly dependent on the orientation of the cameras. To understand the effects and potential benefits of controllable cameras on video analytics, we ran our models on our new PTZ video dataset for each orientation. We then compare the following schemes: 


\begin{enumerate}
    \item \Para{Best fixed orientation per model.} This represents the best results that a fixed-function camera (the standard today) could yield without rotation and zoom. To determine this orientation for each video, we select the orientation that yields the highest accuracy for the model, query, and video.
    \item \Para{Best overall fixed orientation.} This represents the best results that a fixed-function camera could yield without rotation and zoom across all models and queries. This represents a more realistic case where the camera produces frames for some orientation, and all the models and queries run on that same feed.
    \item \Para{Best dynamic orientation per model.} This represents the best results that a PTZ camera could yield by tuning the rotation and zoom knobs on a per-frame basis; this assumes instantaneous orientation changes across frames. We select orientations to produce the highest average accuracy for each video, model, and query.
    \item \Para{Best overall dynamic orientation.} This represents the best results that a PTZ camera could yield by tuning the rotation and zoom knobs on a per-frame basis with the goal of maximizing overall accuracy across all models and queries, i.e., one orientation is used in each frame for all models and queries.

\end{enumerate}
Figures \ref{fig:binary-classification} \ref{fig:count}, \ref{fig:detection}, and \ref{fig:aggregate-count} directly show the aforementioned schemes and how dynamically changing the knobs can drastically improve the performance of the models for binary classification, object counting, and object detection respectively. This is because of the mobility of people and cars that causes object densities to change over time. As a result, the best orientation for the video is not constant and changes over time accordingly to the objects' positions. We further explore the duration that the best orientation remains optimal. In Figure \ref{fig:duration-cdf}, we show that more than half of the time, the best orientation only remains optimal for 1 second, demonstrating that not only does the best orientation change, but also that it changes frequently as the results are highly sensitive to object movements.

Thus, it is clear that the performance of the models is highly dependent on the the specific knob configurations.  Below we break down the improvements achieved from tuning each knob.

\Para{Knob 1: Rotation.} Panning and tilting the camera can bring objects outside of the frame into the field-of-view allowing them to become detected. Figure \ref{fig:rotation1}, shows how panning to the left can find more objects that weren't seen in the original image shown. Further, models' detection abilities can be dependent on not only the object being in the frame, but also the position within the frame it resides in. In Figure \ref{fig:rotation2}, the van cannot be detected in the left image but can be found on the right image after rotating after panning to the left. Lastly, object densities within the scene are dynamic and change over time. Hence, the optimal orientation is not constant throughout the duration of the video and thus the knobs must be continuously reconfigured to maximize query accuracies. For instance in Figure \ref{fig:rotation3}, the original image only contains 3 cars while the image on the right, which features the same scene 1 minute later, contains 5 cars \footnote{For cars, we use an object detection confidence threshold of 0.5 to determine whether a car has been detected. Cars with detection scores below this threshold are ignored.}.

\Para{Knob 2: Zoom.} Models often have difficulties in identifying objects that are far from the camera. By utilizing zoom, the object sizes increase and are thus more easily identified. Further, zooming eliminates many other parts of the scenes from the field-of-view so the objects that are close to the center begin conusming a higher percentage of the frame. In Figure \ref{fig:zoom1}, 2 cars are identified at the bottom of the frame. The right image shows that the zoomed-in photo yields detections for 3 cars in the center that were not identified previously.


Delving deeper, we also find that the amount of improvement yielded from knob tuning varies and is dependent on the models, query types, objects of interest, and scene. That is, the discrepancies between the accuracies for both the best fixed orientations and the dynamically-tuned orientations (i.e., the accuracies reached when knob tuning is used) vary because of different models, query types, object types, and scene that are affected differently from the knobs. For instance, knob tuning improves car counting for Faster RCNN by only x\% while people counting for SSD reaches an improvement of y\%. Below we enumerate on the factors that affects query results.

\begin{enumerate}
    \item \Para{Model architecture.} Due to different architectures, there is variance in how each model is affected by the knobs. For instance, two models may be able to identify an object but only when it's in different positions of the frame. Hence, the orientation that may help one model identify the object may be different from the orientation that helps the other model identify it. Further, larger models (e.g., two-shot detectors such as Faster RCNN) are generally more effective at detecting objects of different sizes and positions. In contrast, lighter weight models (which are quickly becoming more ubiquitous in video analytics deployments due to resource-constrained edge boxes \cite{!!!}) are more reliant on camera knob tuning to optimally position the objects of interest within the frame to compensate for poor performance.
    \item \Para{Query type.} We find that the improvement that can be attained from knob tuning is highly dependent on the coarseness of the query type. For instance, binary classification, our most coarse-grained query, is solely concerned with finding a single instance of an object in the frame. Thus, if there are many objects across different locations in the scene, any orientation that captures at least one of those objects would satisfy the query for that frame. On the other hand, aggregate counting is much more sensitive to the knobs since many objects require the camera to rotate or zoom to find them as they will not be detected in the field-of-view for many orientations.
    \item \Para{Objects of interest.} Improvements also vary by object type used in the queries. Recall that the objects we focus on in this paper are cars and people. Since cars are bigger in size, they are easier to detect. Further, people are generally more dispersed across the scene and can move in many different directions whereas cars are limited to streets and can travel in fewer different directions. Thus, there's more variance in the optimal orientation for people.
    \item \Para{Scene.} Due to the diversity of our video dataset, there is a lot of variance in object positioning, movement, and quantity. Frames that feature fewer objects that are clustered together provide little opportunity for controllable cameras to improve upon the performance yielded from traditional static cameras. At the other end of the spectrum, frames with many objects that are widely dispersed throughout the scene provide ample opportunity for controllable cameras to achieve significant improvements over static cameras. Further,   the presence of other elements in the scene such as lighting or trees in the background, can either positively or negatively influence the models' results despite not directly affecting the size or view of the objects of interest. Additionally, movement can play a significant role since an object that is moving at a high speed the object can be missed altogether if inference is running too infrequently.
\end{enumerate}


With that said, it is clear that while the usage of knobs can produce higher query performance over traditional fixed cameras, they must be tuned carefully because of the large amount of sensitivity they have on the query results. This is further complicated by not only the existence of the aforementioned properties of the analytics pipeline influence that can optimal orientation at any time, but also that multiple models and queries are used on the same frames. In the next section, we delve into our online approach to automatic camera knob tuning to improve query performance whilst balancing these considerations.

%  Figure \ref{fig:accuracy-degradation} shows the model degradations observed when a model adopts the optimal camera orientations for other models demonstrating that models react differently to the knobs. That is, one model will benefit from a different set of knob settings than the others.




==> motivation2.tex <==
\section{Background and Motivation}
\label{s:motivation}

\subsection{Overview of Live Video Analytics}
- describe the general pipelines: videos are streaming to edge or cloud servers, and CNNs run on each one to generate results

- pipelines goal is to meet accuracy target: query developers or app set this, and goal of pipeline is to generate sufficiently accurate results with as low resource usage as possible

- 4 query types (and accuracy definitions) [note that privid handles aggregate counting queries]; workload is composition of these

- Related work covers enhancements for accuracy and resource efficiency. work assumes a set of video streams, and there are three classes of techniques: (1) tune pipeline/server-side knobs, (2) filter unnecessary frames/streams, (3) compressed models

\subsection{Importance of Tuning Camera Configurations}

- results here use the same datasets and methodology in eval; briefly, it considers a handful of models and the query types from 2.1, and regions of interest in the 360-degree videos (that are cut into grids). In each video, we obtained query/workload results for all possible orientations at each time, and defined accuracy relative to the 'best' orientation at each time, i.e., the orientation that maximized accuracy. For instance, for a binary classification query considering cars, all orientations that have a car (as per the query/model) would be considered the 'best' orientations and deliver accuracy of 100\%; all other orientations would yield accuracy of 0\%. In contrast, for counting/detection, the 'best' orientation(s) would be the one(s) with the max number of relevant objects, and accuracy for any orientation would be its count over that max count (or mAP for detections). For aggregate counting, the best orientation is not a time-instant decision, and instead is based on previous and future decisions; due to compute constraints, we approximate this by estimating the best orientations at any time using a time-instant metric that does the following: we weight each orientation by the number of previously-unseen objects it possesses, weighted by how often the object will appear again (at any orientation) later in the video (this is a proxy for the likelihood that we'll find it later); testing on a few videos, we find that this picks the best dynamic X\% of the time compared to the true optimal. From these results, we draw several important conclusions, described in turn. For space, we show results for representative queries and workloads in our eval; eval shows results for all, and we note that all presented trends hold for all.

(1) for a given workload, the  best orientation changes rapidly over time
- graph with CDFs for all queries/workloads and videos that show how often orientations remain best
- graph showing the accuracy implication of not adapting to the changing 'best orientations'. Three CDF curves: best dynamic (changing frequently), one-time static which picks the best at the beginning and keeps it, and best fixed. Even if we had (unrealistic) a priori knowledge and picked best fixed, it still leaves a lot on the table [comment on the trends, e.g., coarser queries like binary classification have smaller gaps between best fixed/best dynamic, while agg counting will be high!]
- graph showing that many orientations are best for a short amount of time, so they are important for accuracy but it would be wasteful to dedicate a new camera to that specific orientation. graph can be distribution of duration as 'best' for top k orientations.

(2) at any time, the best orientation can vary wildly for different queries/workloads
- clustered bar chart showing what happens accuracy-wise if you apply the best dynamic orientations according to one query/workload, to others (relative to applying their best dynamic orientations). [could do this for best fixed, but that seems silly since we just showed that best dynamic is better]

%Taking a step back, there are two reasons for this behavior:
%- new objects enter the scene
%- existing objects move around (or the scene generally changes) and are thus presented differently (and perceived differently) by the models
% perhaps approximate relative impact of each using dedup techniques? otherwise, what's the point of bringing this up?

%There are two reasons for this:
%(1) fairly obvious, but the scenes change! -- do we need to show this? if so, we could show heat maps or something over time?
%(2) more interesting though, is that each model and query type exhibits a different sensitivity to the relative position/size of an object in a scene, and thus to orientation changes. 

%[Is there a way to tease out the impact of each of these things? I guess the "single workload over time" speaks to the scene changes, while the "different workloads at one time" speaks to the different sensitivities and the scene changes (since the models are looking for different things)? Maybe we could also show some 


Section 2: Background and Motivation
- quick overview of live video analytics (can also touch on the general approaches to improve efficiency: tune server-side knobs, filter unnecessary content on a per-camera basis, use compressed models)
- "Importance of Camera Configurations" and should just highlight the accuracy wins that come from tuning orientations (best dynamic vs. best fixed). Could show this for individual queries, and then show it for some workloads. Perhaps we could also show examples of what is happening: can be because new objects enter scene or because existing content moves (objects, background) [i.e., for even singular queries, show new objects entering a grid and not being currently visibile but changing the 'best orientation', and show cases where changes in existing object lead to model not detecting the object (don't discuss sensitivities and different model biases)] -- if we can quantify how often each happens, even better!


Section 3: Our approach
- Opportunity with PTZ cameras: describe PTZ cameras (let us rotate/zoom remotely). Give some background about compute they have, etc. High level approach is to simply use these APIs to tune cameras to maximize accuracy. In theory, PTZ cameras can rotate/zoom fast enough to switch between the best dynamic orientations above, so we should be able to reap those accuracy wins.

- Challenges
(1) rapid changes: show results of how often best dynamic changes (how long orientations last as best orientations)
(2) sensitivity: show results of how the best orientations are different for different workloads/queries. then dive into the sensitivities a bit
(3) the search space is massive: while the PTZ camera can be in the best dynamic orientation at any time, it cannot cover all orientations at all time, so we need a search strategy despite the fact that the best orientation changes so quickly
(4) limited network/compute resources: cameras cannot run workloads directly, and also can't send too many frames since network/backend can't support it

S4: Design
- overview: main insight is that PTZ cameras can rotate faster than results are needed, so we can opt for an exploration strategy that is based directly on content in different orientations, rather than purely guesses about what each orientation may have. Building on this, MadEye employs a split architecture whereby cameras employ (1) a search algorithm to determine the orientations to explore at any time (between when results are needed), and (2) a frame selection strategy to pick frames to send to the backend for full workload inference. Server inference results are continually fed back into the camera's algorithms to guide the strategies for both questions (as hints of which orientations were best and also as model updates). We describe MadEye in terms of these two components.

- Search module for exploring orientations
* amorphous search (server-side does profiling of model/query sensitivity and shares that info with client; then algo is client-side and is based on local changes and gradual movement)

- Prioritizing orientations for inference
* continual learning (server bootstraps model training upon registration, clients run model as rankers, and servers periodically train the models and share new copies with clients). much of this will be about model structure (and rationale), how retraining works, the fact that we use per-query/model+orientation cheap models rather than one for the whole thing, etc.


S5: Implementation

S6: Eval

S7: Related Work

S8: Conclusion

--- old below ----


S2: Background and Motivation
- background
- agg results showing need to change orientations




S3: Approach: PTZ Cameras
- overview PTZ cameras
- approach and promise: if you knew where to go, PTZ camera can keep up -- could theoretically match best dynamic from S2
- The main difficulty in achieving this is that the PTZ camera cannot know exactly where to go at all times, and it cannot capture images of all places at all times. This is complicated by several things:
- too many options (large search space)
- different queries/models have different sensitivities to knobs and prefer to be in different orientations
- 


- challenges
* massive search space (can't consider everywhere at all times; we can reach where we need to go only if we know it!)
* sensitivity of queries/models
* rapid changes: need to make quick decisions
* limited network and compute resources: cameras can only do limited compute; can only send limited frames to server at any time




==> paper_outline.tex <==
- Video analytics matters, and lots of work has focused on optimizing resource efficiency and accuracy for already-deployed cameras (e.g., by tuning pipeline knobs). However, deployment is tough too as you must figure out location and orientation of camera. Changing this is practically difficult, and yet analytics queries are highly sensitive to this both based on model biases (and sensitivity to orientation) and object dynamism. Worse, analytics pipelines are often run in wireless or edge settings with limits on network bandwidth, and are presented with diverse queries/models that are sometimes difficult to predict (if it is bring-your-own model). You could deploy tons of fixed cameras for a region, but this is impractical both from a deployment perspective (space/energy) and resource requirements (streaming frames from all of those cameras would be too costly); even with filtering techniques, data would have to be streamed to compare data across orientations. [maybe this should emphasize deploying and configuring cameras] [note that we focus on configuring cameras rather than where in a scene to place them since that is often restricted by things like where poles are, power sources, etc.]

- We study if PTZ cameras can help alleviate this burden. ptz cameras let you tune rotation/zoom remotely, and now cost roughly the same as other cameras. Thus, on the surface, ptz cameras offer a logical solution: deploy one camera for a region and adapt its orientation based on the scene/query. Indeed, our results show that, if done perfectly, this can yield accuracy boosts of X\% compared to even the best fixed/static deployment (that is unrealistic to achieve).

- However, realizing this is tough for a few fundamental reasons:
(1) each different query type/model pair exhibits a different sensitivity to configuration knobs (rotation/zoom) - some summary number
(2) the environment is non-stationary and unpredictable (perhaps show how best orientation changes rapidly?)
(3) the search space of orientations is large (even for a small region), and yet, the camera must respect network and backend compute restrictions (it can't just send all orientations all the time)

These reasons collectively preclude prior search algorithms for non-stationary environments (e.g., multi-armed bandits) that aim to predict the importance of a given orientation (and thus when to revist it) based on a past visit to it. The issue is that the importance of each orientation changes too rapidly for this to work.
*** somehow, we should bolster the sensitivity study a bit since that is itself new IMO; I don't think others have studied the sensitivity of models to these knobs!

To fill this void, we built MadEye, a system that delivers continual and resource-efficient video analytics with high accuracy. The key insight behind MadEye is that the speed at which PTZ cameras can now rotate (e.g., 400 degrees per second) far outpaces the rate at which analysts require results (often 1 FPS – see focus and other papers). This, in turn, allows MadEye to eschew the predictive approaches above and instead employ a scheme that rapidly captures a bunch of images for different orientations at a given time (i.e., between inferences), and based on their actual content, determine which are the most fruitful, i.e., which would maximize accuracy for a given workload and bandwidth availability. MadEye embeds several new techniques to realize this idea.

(1) determining which orientations to consider at any time (even with rotations, we can't cover them all)
- not sure what the ideas/insights are here since we no longer have to worry about local vs. distant switches? perhaps the insight still holds? i.e., that best orientation changes are often local? except here, local would kinda be the center of the previous region? in essence, we have an amorphous region, and we sort of try to keep it relatively stable at the core, but are willing to *gradually* move in different directions?

(2) picking the best orientation(s) from the considered set
- can't run the whole workload at the edge, so we simplify this to a much simpler rank problem
- lightweight continual learning: harder problem than the past for continual learning (which was just classification of pre-determined bounding boxes). instead, we have to rank the different options in terms of accuracy for given workload. Key idea is to structure this as a much simpler problem for the model (so we can get away with using a really cheap model): don't use a ranker that takes in a bunch of images, and instead, predict counts for each image alone, and then rank based on those counts. note that we don't need perfect counts; just enough to get the right rankings. We choose this because loss functions for tasks like counting are much easier to use than those for ranking (why??)
- the use of count as a proxy for different queries is interesting -- why is this okay?
- the model is trained periodically using the real workload results only for images that are actually sent to the backend (so there is no additional full-workload inference that we are introducing)
- explain how this cheap model is meant to just sufficiently approximate each model in the workload (is it meant to find count of all relevant objects?)

(3) ?????? -- could be something about multi-camera?


- Evaluating PTZ cameras requires a dataset that allows the tuning of rotation and zoom at every time instant, i.e., we cannot use a dataset that is based on specific rotation/zoom decisions, and instead need the ability to tune those knobs ourselves. To our knowledge, such a dataset does not exist. So, we created one using publicly available 360-degree videos. We divided them into an overlapping grid (to mimic a continual rotation space), and enable zoom using ??? 

- Using this dataset, we evaluated MadEye on a variety of deep learning models and query types: classification, counting (both per frame and aggregate), and detections, as well as different network conditions. Across these scenarios, MadEye is consistently and continually able to meet accuracy targets. Specifically, MadEye achieves X-Y\% accuracy boosts compared to the (impractical) best fixed camera approach; results are Y-Z\% relative to the unachievable best PTZ approach. More practically, accuracy boosts are Y-Z\% and Z-Y\% relative to existing PTZ tracking algorithms, and Z\% over generic multi-armed bandwidth searches. Framed differently, to achieve the same accuracy, MadEye requires Y-Z\% fewer cameras and bandwidth relative to the best possible approach of deploying fixed cameras. We will open source. [could also tease out whole scene and aggregate stuff as things that become more reaslistic with PTZ]

In summary, our contributions are:
- sensitivity study to this emerging class of knobs
- Madeye, system that efficiently and automatically explores regions using PTZ cameras to enable high-accuracy analytics under bandwidth constraints, thereby simplifying the camera deployment challenge for operators. MadEye uses a novel continual learning strategy to guide its search.
- A thorough evaluation of MadEye with different models/queries, and a new dataset (which is required when considering rotation/zoom) that we will release.



_______intro notes______

maybe this should really just focus almost entirely on small regions (wanting to do analytics on an intersection or a part of a street): even in that small area, there are tons of orientations. objects move and models are sensitive, and so a fixed camera will surely miss many things (since the right orientation will vary over time). PTZ lets you cover that area with just one camera.
* and then we can say, this naturally extends to broader scenes (the results scale as expected), and also the wins grow for other types of queries like aggregate counting
* for a small region, how many orientations are there? 


we are improving accuracy per bandwidth: you would have to deploy many fixed cameras to cover important regions and orientations, but 


you could deploy tons of fixed cameras, but then you'd still have the challenge of figuring out which set of frames to send to best use available bandwidth! Each can do local computations, but that is not enough.


_______________Section 2: Background and motivation____________

2.1: background of video analytics that describes queries (CNNs, types of queries, accuracy definitions, and general goals).

2.2: the problem: deploying/configuring cameras for high accuracy is challenging [or perhaps simplify to configuring cameras?]
- results here use the same datasets and methodology in eval; briefly, it considers a handful of models and the query types from 2.1, and regions of interest in the 360-degree videos (that are cut into grids)
- main points:

(1) for a given workload, best orientation changes rapidly over time
- CDFs for all queries/workloads and videos that show how often orientations remain best
- graph showing what happens accuracy-wise if you are only willing to adapt (i.e., change best orientation) at certain frequencies -- less often should be lower accuracy and if you compare with very frequent, it shows how much accuracy is being left on the table

(2) at any time, the best orientation can vary wildly for different queries/workloads
- clustered bar chart showing what happens accuracy-wise if you apply the best orientation for one query/workload to other queries/workloads (relative to applying the correct best orientations in each case). Two versions: one picks best orientations using best fixed, while the other is using best dynamic

There are two reasons for this:
(1) fairly obvious, but the scenes change! -- do we need to show this? if so, we could show heat maps or something over time?
(2) more interesting though, is that each model and query type exhibits a different sensitivity to the relative position/size of an object in a scene, and thus to orientation changes. 

[Is there a way to tease out the impact of each of these things? I guess the "single workload over time" speaks to the scene changes, while the "different workloads at one time" speaks to the different sensitivities and the scene changes (since the models are looking for different things)? Maybe we could also show some 

One solution could be to place more cameras, but this poses a resource challenge since the scenarios are often network constrained, and yet determining how best to use the limited network resources requires shipping and co-analyzing the frames from each camera at any time. 



Section 3

==> ptz.tex <==
\section{Our Approach: PTZ Cameras}
\label{s:ptz}


- Results in previous section highlight the importance of adapting camera configurations. The need stems from two patterns: new objects entering the scene and existing objects (or their surroundings) moving. In either case, our goal is to re-orient cameras to capture the maximum number of relevant objects at any time, i.e., bringing new objects into view, and continuing to locate/identify previously seen objects.

- PTZ cameras afford such dynamism. [Describe their APIs in more detail, on-camera compute resources, etc.] However, existing approaches don't make sense here (tracking objects). Instead, we must take a query/model-centric approach. We do sensitivity study here.

- 


